Machine learning of a density functional for anisotropic patchy particles

Anisotropic patchy particles have become an archetypical statistical model system for associating fluids. Here we formulate an approach to the Kern-Frenkel model via classical density functional theory to describe the positionally and orientationally resolved equilibrium density distributions in flat wall geometries. The density functional is split into a reference part for the orientationally averaged density and an orientational part in mean-field approximation. To bring the orientational part into a kernel form suitable for machine learning techniques, an expansion into orientational invariants and the proper incorporation of single-particle symmetries is formulated. The mean-field kernel is constructed via machine learning on the basis of hard wall simulation data. Results are compared to the well-known random-phase approximation which strongly underestimates the orientational correlations close to the wall. Successes and shortcomings of the mean-field treatment of the orientational part are highlighted and perspectives are given for attaining a full density functional via machine learning.

==> _region_.tex <==
\message{ !name(master.tex)}
\message{ !name(merged.tex) !offset(44) }

\title{Machine learning of a density functional for anisotropic patchy particles }
\author{Alessandro Simon}
\affiliation{Institute for Applied Physics, University of Tübingen, Germany}
\affiliation{Max Planck
Institute for Intelligent Systems, Tübingen, Germany}
\author{Jens Weimar}
\affiliation{Institute for Applied Physics, University of Tübingen, Germany}
\author{Martin Oettel}
\affiliation{Institute for Applied Physics, University of Tübingen, Germany}

\begin{abstract}
    Anisotropic patchy particles have become an archetypical statistical model system for associating fluids. Here we formulate an approach to the Kern--Frenkel model via classical density functional theory to describe the positionally and orientationally resolved equilibrium density distributions in flat wall geometries. The density functional is split into a reference part for the orientationally averaged density and an orientational part in mean field approximation. To bring the orientational part into a kernel form suitable for machine learning techniques, an expansion into orientational invarinats and the proper incorporation of single-particle symmetries is formulated. The mean field kernel is constructed via machine learning on the basis of hard wall simulation data. \tr{Results are compared to the well-known random-phase approximation and show clear deviations...?}
    Shortcomings of the mean-field treatment of the orientational part are highlighted and perspectives are given for attaining a full density functional via machine learining.  
\end{abstract}
\maketitle
\section{Introduction}

A useful model system for describing various phenomena in soft matter physics is given by patchy particles where particles with an isotropic repulsive core additionally interact via a certain number of attractive bonding sites distributed over their surface. These patchy particle systems show novel phenomena such as the existence of empty liquids \cite{bianchi_phase_2006, heras_phase_2011} or of stable equilibrium gels \cite{smallenburg_liquids_2013, sciortino_equilibrium_2017}. The Kern-Frenkel (KF) model is an example for such a patchy particle model with a mathematical form for the pair potential which is easy to simulate \cite{kern_frenkel2003}. In fact, many theoretical insights have been obtained by simulations \cite{foffi2007possibility,romano2010phase}. An alternative approach to simulations for obtaining equilibrium properties of soft matter model systems is (classical) density functional theory (DFT). It has been frequently and successfully employed for isotropic fluids \cite{lutsko2010recent,evans2009density}, in particular for hard particles in the form of the very precise fundamental measure theory (FMT), for a review see Ref.~\cite{roth2010fundamental}. For the specific case of patchy particles, FMT-based functionals have been derived \cite{yuwu2002,stopper2018bulk} which are functionals of the \textit{orientationally averaged} density profile. These functionals describe various properties of patchy particles reasonably well (e.g. phase diagrams and orientationally averaged pair correlations), but there are limitations which are clearly due to the neglect of orientational correlations (e.g. density profiles around hard tracer particles). Thus it is desirable to find free energy functionals of the full orientation-dependent density profile. However, there are no analytical methods known to construct of such functionals for anisotropic particles which are similar in accuracy such as FMT for hard particles. Hence it appears to be promising to turn to numerical and data-driven methods such as machine learning (ML) for this task.               

Finding classical density functionals with ML methods is a rather recent development. Initial work has focused on model fluids in one dimension (1D) \cite{shang2019classical,shang2020FEQL,yatsyshin2021,wu2022}, whereas work on more realistic systems in 3D is scarce, for a study of the 3D Lennard-Jones (LJ) fluid see Ref.~\cite{cats2021}. Among these works one can distinguish between approaches to learn integral kernels for the generally unknown, but sensibly parametrized part in the functional describing attractive interactions \cite{shang2019classical,cats2021}, an approach to learn an analytic expression for the entire functional \cite{shang2020FEQL} and studies more focussing on the uncertainty assessment of the learned density functional maps \cite{yatsyshin2021,wu2022}. The ML literature on density functionals for the quantum electron problem goes back a few more years \cite{burke2012}, recent developments show interesting parallels to the approaches taken for classical systems, as e.g. a work on finding analytic functionals in \cite{lili2022} or the use of the minimizing equations in the ML networks \cite{lili2021}. 

In this paper, we am at finding a density functional for the KF model with ML methods, describing the orientational correlations from Monte Carlo simulation data between hard walls. The approach is similar in spirit to Refs.~\cite{shang2019classical,cats2021} in that an \textit{ansatz} for the unknown part in the functional is chosen which employs weighted densities and ML is used to  M. Wertheim, Thermodynamic perturbation theory of
polymerization, The Journal of chemical physics 87, 7323
(1987determine these weights. We restrict our \textit{ansatz} to a mean field form where the learned weights have a straightforward interpretation and may be compared to standard forms from liquid state theory. We note that mean field forms have been employed before in DFT studies of anisotropic particles, see Refs.~\cite{cattes2016,wandrei2018mean} for a Heisenberg-type fluid where the mean field form is directly taken from the anisotropic, attractive part of the interaction potential (random-phase or RPA approximation), or Ref.~\cite{teixeira2019patchy} for a patchy particl M. Wertheim, Thermodynamic perturbation theory of
polymerization, The Journal of chemical physics 87, 7323
(1987e fluid with two patches where the mean field part is simply assumed. The present study, in contrast, introduces a sensible method to obtain an "optimized" mean field form for the orientational part of the density functional, constrained by simulation data. For anisotropic fluids, even simple mean--field functionals are technically challenging: the density depends on six variables, 3 spatial coordinates and 3 orientation angles. A systematic expansion of the orientational part proceeds via Wigner D-matrices and orientational invariants, pioneered in integral equation studies of anisotropic fluids \cite{blum1972invariant} and developed more recently in the context of integral equation and DFT studies of water in refs.~\cite{ding2017efficient,belloni2017exact,jeanmairet2013molecular,borgis2021accurate}. 
This expansion allows also controlled truncations. Nevertheless, to make the problem suitable for machine learning, some basic formalism regarding the orientational expansion and the proper incorporation of single-particle (molecular) symmetries) needs to be laid out which (besides the actual machine learning of the mean field functional) is one of the main aims of the present paper.    
We hope that the method can be extended in the future to tackle the task of finding the ``full'' functional for patchy and other anisotropic particles.     

The paper is structured as follows: ...


\section{Theory}
\subsection{Kern-Frenkel potential}


The KF fluid we consider is modelled by a hard sphere with four attractive patches placed at the corners of a tetrahedron which is centered in the middle of the molecule. 
Besides the tetrahedron condition (angle between patch vectors equal to  $\arccos ( -1/3)$) one is still free to chose the exact placement of the patches in the molecule's body-fixed reference frame. Depending on this convention, the symmetry conditions 
in terms of the Euler angles change, which can be useful later on. Two popular choices are the following:

\paragraph*{Convention A}

Here the patches are placed at the following positions
\begin{equation}
P_A = \frac{1}{\sqrt{3}}\begin{pmatrix}
  -1& 1 & 1 & -1\\
  -1 & 1 & -1 & 1\\
  1 & 1 & -1 & -1
\end{pmatrix}  
\end{equation}
where each column $\alpha$ is a unit vector $\hat{\bm{r}}^{\alpha}$ pointing from the center to the patch. All vector components have
the same magnitude and it is rather easy to see which mirror symmetries the molecule posseses.



\paragraph*{Convention B}

We rotate the configuration from the previous convention by the angle $\frac{\pi}{4}$ (actively) around the $z$ axis to get convention (B). Here, a pair of patches
is placed along the $xz$ plane, while the other pair sits on the $yz$ plane.
The positions are
\begin{equation}
  P_B = \frac{1}{\sqrt{3}}\begin{pmatrix}
    -\sqrt{2} & \sqrt{2} & 0 & 0\\
    0 & 0 & -\sqrt{2} & \sqrt{2}\\
    1 & 1 & -1 & -1
  \end{pmatrix}  
  \end{equation}
The reason we prefer this convention is that two symmetry planes fall together with the coordinate planes. 
In principle, however, any choice is permissible.




 
\begin{figure}%
  \centering
  \subfloat[\centering Convention (A)]{{\includegraphics[width=0.7\columnwidth]{ref1.png} }}%
  \qquad \qquad
  \subfloat[\centering Convention (B)]{{\includegraphics[width=0.7\columnwidth]{ref2.png} }}%
  \caption{The two conventions that are used for the placement of the patches in the body-fixed system.}
  \label{fig:example}%
\end{figure}

{The KF potential between a pair of molecules is a sum of a hard sphere part $\phi_\text{HS}(r)$ for diameter $\sigma$ and
an anisotropic patch part $V^\text{KF}$ which  depends on the individual orientation of the molecules} and their
positions relative to each other. For parameterizing the orientation of a three dimensional body
we will use the well known Euler angle parameterization with the angles
$(\phi, \theta, \chi) \equiv \Omega$ and 
\begin{equation}
 \int d\Omega:= \int_0^{2\pi} \odif{\phi} \int_0^\pi \odif{\theta} \int_0^{2\pi} \odif{\chi} = 8 \pi^{2} =: K.    
\end{equation}



The anisotropic part of the potential is defined by
\begin{equation}
  \label{eq:16}
  V^\mathrm{KF}(\bm{r}_{12}, \Omega_{1}, \Omega_{2}) =  \phi_{\mathrm{sw}}(r_{12}) \sum_{\alpha,\beta=1}^{N_\text{p}}  \phi_{\text{patch}}(\bm{r}_{12}, \hat{\bm{r}}_{1}^{\alpha}(\Omega_{1}), \hat{\bm{r}}_{2}^{\beta}(\Omega_{2}))
\end{equation}
Here, $N_\text{p}$ is the number of patches and   $\phi_{\text{sw}}(r)$ is a square well potential
\begin{equation}
  \phi_{\text{sw}}(r)~=~ \left\{ \begin{matrix} -\epsilon \qquad (r \in [\sigma,\sigma+\delta]) 
      \\ 0 \qquad \text{(otherwise)} \end{matrix} \right.
\end{equation}
with the attractive range $\delta$ and attraction depth $\epsilon$. $\phi_{\text{patch}}$ is the orientational patch-patch part
\begin{equation}
  \label{eq:17}
  \phi_{\text{patch}}(\bm{r}_{12}, \hat{\bm{r}}_{1}^{\alpha}(\Omega_{1}), \hat{\bm{r}}_{2}^{\beta}(\Omega_{2}))  = \begin{cases}
    1 &\text{if}\quad\begin{cases}
      \hat{\bm{r}} \cdot \hat{\bm{r}}_{1}^{\alpha} > \cos \theta_{\text{max}}\\
      -\hat{\bm{r}} \cdot \hat{\bm{r}}_{2}^{\beta} > \cos \theta_{\text{max}}
    \end{cases}\\
    0 &\text{else}
    \end{cases}
  \end{equation}
characterized by the opening angle $\theta_{\text{max}}$ of the ``cones" that interact attractively between the particles. 
{Here, $\bm{r}_{12}=\bm{r}_{1}-\bm{r}_{2}$ is the vector connecting the two centers of the particles, and $\hat{\bm{r}}_i^{\alpha}$ is a unit vector from the  center  of  particle $i$ to  a  patch $\alpha$ on  its  surface  depending  on  the  particle orientation $\Omega_i$.}
In general, depending on the chosen parameters,
more than two patches could be bonded. For certain choices of $\delta$ and $\theta_\text{max}$ 
this is avoided (single bond condition) and this will be adopted in the actual calculations, see below.


\subsection{Expansion of the density distribution}

Owing to the orientational dependence of the density distribution on three angles, its behavior could be rather complex and visualizations are not easy. The complexity is reduced by expanding the 
orientational part in a suitable functional basis, the Wigner D-matrices $\wD^l_{mn}(\Omega)$ \cite{rose1995elementary, gray84theory}
These are given by
\begin{equation}
  \label{eq:15}
  \wD^{l}_{mn}(\phi, \theta, \chi) = e^{-i m \phi} d^{l}_{mn}(\theta) e^{-i n \chi}
\end{equation}
with the integer indices $m,n$ running from $-l$ to $l$ and $l \in \mathbb{N}$.
Then, the forward and backward transformation of a sufficiently well behaved function $f$ that may depend also on other variables, here $\bm{r}$, are given by
\begin{gather}
  f(\bm{r}, \Omega) = \sum_{lmn} f^{l}_{mn}(\bm{r}) \wD^{l}_{mn}(\Omega) \label{eq:d_expansion}\\
  f^{l}_{mn}(\bm{r}) = \frac{2l + 1}{K} \int \odif{\Omega} f(\bm{r}, \Omega) \conj{\wD^{l}_{mn}}(\Omega)  \label{eq:expansion_coeff}\;,
\end{gather}
{where $\conj{\wD^{l}_{mn}}$ is the complex conjugate of $\wD^{l}_{mn}$.}
We call $f^{l}_{mn}$ the (orientational) moments of the function $f$.%

We adopt {Euler angles in the $zyz$ prescription for describing rotations of the molecule.} Explicitly, the body-fixed reference frame is first rotated by the 
angle $\phi$ around the original $z$ axis, resulting in two new perpendicular axes $x'$ and $y'$. Then we rotate the frame by the angle $\theta$ around
$y'$, resulting again in two new axes $x''$ and $z''$, while $y'' \equiv y'$. The final rotation of $\chi$ is done around $z''$. The order of these operations is also 
reflected in the arguments of the D-matrix. Alternatively, the same rotation can be achieved by rotating around space-fixed axes $XYZ$ with the
same angles but in reverse order, i.e. by $\chi$ around $Z$, then by $\theta$ around $Y$ and then finally by $\phi$ around $Z$ again.


\subsubsection{Symmetry constraints}

The existence of symmetries lead to certain moments in the above expansion to vanish or to become linearly dependent.
Two kinds of symmetries arise in our context. Firstly, due to the symmetry of the molecule and the indistinguishability of the patches, a certain rotational configuration
$\Omega$ might be physically equivalent to another configuration $\Omega' \neq \Omega$. This is the molecular symmetry, in our case the (chiral or rotational)
tetrahedral group $T$, containing 12 elements. The full tetrahedral $T_d$ group also includes reflections and contains 24 elements in total.
The groups $T$ and $T_d$ are isomorphic to the alternating group $A_4$ and the symmetric group $S_4$, respectively. Thus it is possible to 
label the symmetry rotations of the tetrahedral group with the permutation of the four corners of the tetrahedron.

Secondly, the external potential may also introduces additional symmetry constraints on the density and orientation distribution. In our case of an orientation-independent flat wall potential this will be an additional rotational symmetry perpendicular to a wall normal, see below.

For treating the molecule symmetry, we adapt the exposition in ref.~\cite{steele1980symmetry} to our purpose.
Suppose the function $f(\Omega)$ is invariant under the group $G$, that is
\begin{equation}
  \label{eq:invariance_f}
  f(\Omega) = f(\Omega') = f(\Omega'') = \cdots
\end{equation}
where the primed orientations correspond  to orientations ``congruent'' to the initial one and result from acting on $\Omega$ with one group element $g \in G$. This is equivalent to permuting the patches before bringing the molecule to orientation $\Omega$.
Each of the previous $f(\cdot)$ can be expanded into Wigner matrices as in eq.~\eqref{eq:d_expansion}.  $D(\Omega')$ is related to $D(\Omega)$ through a transformation law for
Wigner matrices under rotation of the body-fixed axes, 
\begin{equation}
\wD^l_{kn}(\Omega') =  \wD^l_{kn}(\Omega R) = \sum_{m} \wD^l_{km}(\Omega)  \wD^l_{m n}(R),
\end{equation}
see, e.g., Ch. 4.7, eq. (1) in \cite{varshalovich1988quantum}, or eq. (A.101) in~\cite{gray84theory}. 

Note, that here the Wigner matrix serves in principle two purposes. Once it is used as a basis for $f \in L^2(\mathrm{SO}(3))$
and a second time for rotating these basis functions.
We can now sum over all the terms in eq.~\eqref{eq:invariance_f} and divide by the number of symmetry elements $|G|$ arriving at
\begin{equation}
  \label{eq:7}
  \frac{f(\Omega) + f(\Omega') + \cdots}{|G|} = f(\Omega)
\end{equation}
Expanding both sides in the Wigner basis leads to the following condition
\begin{multline}
  \label{eq:5}
  {\sum_{lmn}} f^l_{mn} \wD^l_{mn}(\Omega)  \\ =  {\sum_{lmn}} f^l_{mn} {\sum_k}\wD^l_{mk}(\Omega)  \frac{1}{|G|} \sum_{R_i \in G} \wD^l_{k n}(R_i) \\ 
  =
  {\sum_{lmn}} f^l_{mn} {\sum_k} \wD^l_{mk}(\Omega)  \pOp^{(l)}_{kn}
\end{multline}
where we define the projection operator as
\begin{equation}
  \label{eq:proj_op}
 \frac{1}{|G|}  \sum_{R_i \in G} \wD^l_{k n}(R_i) =   \pOp^{(l)}_{kn}
\end{equation}
In eq.~\eqref{eq:5}, one can project onto the moments $f^l_{mn}$ by applying $(2l+1)/K \int d\Omega \conj{D^{l'}_{m'n'}} \cdots $ to both sides. We obtain:
\begin{equation}
  \label{eq:8}
  f^l_{mn} = f^l_{mk} \pOp^{(l)}_{nk}
\end{equation}
which corresponds to a linear equation for every row of the coefficient matrix $f^l_{mn}$, written in the usual form as
\begin{equation}
  \label{eq:9}
  \pOp^{(l)}_{nk} f^l_{\circ k} = f^l_{\circ n}
\end{equation}
Solving this equation leads to the sought symmetry conditions of the expansion coefficients.


This is equivalent to the fact that not every Wigner matrix can appear in the expansion of an invariant function. Just like the function itself, the basis functions that appear must also be invariant and this can only be achieved by certain linear combinations of Wigner matrices. We can write the new, symmetric basis as
\begin{equation}
  \label{eq:27}
  \Delta^l_{m}(\Omega) = \sum_{n} d^l_n \wD^l_{mn}(\Omega)
\end{equation}
Repeating the above calculation for the invariant $\Delta^l_{m}(\Omega)$ instead of
the $f(\Omega)$ leads to the same linear equation, only this time with the interpretation of having constructed a $G$ invariant
basis of $L^2(\mathrm{SO}(3))$. The resulting eigenvalue problem is similarly
\begin{equation}
  \label{eq:30}
\sum_k    \pOp^{(l)}_{nk} d^l_{k} = d^l_{n}
\end{equation}
In principle there could be $2l+1$ orthogonal eigenvectors for every value of $l$ (imagine the case without any symmetry) but usually the number of
eigenvectors with eigenvalue $1$ is much smaller. We will therefore label the solutions by an index $j$
as in 
\begin{equation}
  d^l_{[j]n}
\end{equation}
such that we can also label the basis functions accordingly
\begin{equation}
  \Delta^l_{m[j]}(\Omega) = \sum_{n} d^l_{[j]n} \wD^l_{mn}(\Omega)
\end{equation}
In order for the new basis function to fulfill the same normalization as the Wigner matrices one needs to scale the $d^l_{[j]}(n)$ such that
\begin{equation}
\sum_n \Bigl(d^l_{[j]n}\Bigr)^2 = 1
\end{equation}

\begin{table}
\begin{center}
  \begin{tabular}{cccc|ccc} 
  \toprule
  permutation & $\phi$ & $\theta$ & $\chi$ &$\phi$&$\theta$&$\chi$  \\
  \midrule
  (id) & 0 & 0 & 0 & 0&0&0\\
  (012) & 0&$\pi/$2&$-\pi/2$ &$ -\pi/4$&$ \pi/2$& $-\pi/4$\\
  (031) & $\pi$& $\pi/2$&$\pi/2$ &$3\pi/4$&$ \pi/2$&$ 3\pi/4$ \\ 
  (132) & $\pi$& $\pi/2$&$-\pi/2$ &$ 3\pi/4$& $\pi/2$&$ -\pi/4$\\ 
  (023) & 0& $\pi/2$&$\pi/2$ &$-\pi/4$& $\pi/2$&$ 3\pi/4$\\  

  (021) &$-\pi/2$ & $ \pi/2$ & $\pi $& $-3\pi/4$ & $ \pi/2$ & $ -3\pi/4$\\ 
  (013) &$ \pi/2$ & $\pi/2$ &0 &$ \pi/4$& $\pi/2$&$ \pi/4$\\ 
  (123) &$ -\pi/2$& $\pi/2$&0 &$ -3\pi/4$&$ \pi/2$&$ \pi/4$\\ 
  (032) &$  \pi/2$& $\pi/2$&$\pi$ &  $\pi/4$& $\pi/2$&$ -3\pi/4$\\
    
  (02)(13) & 0&$\pi$&0 &$ -\pi/2$& $\pi$& 0\\
  (01)(23) & $\pi$&0&0 & $-\pi$& 0& 0\\ 
  (03)(12) & $\pi$&$\pi$&0 &$\pi/2$& $\pi$& 0 \\
  \bottomrule
  \end{tabular}
  
  \caption{\label{tab:angles_T}Angles for the rotations in the group $T$ for two different conventions of the body frame }
  \end{center}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{ccc}
\toprule
  $l$ & non-zero & independent \\
    & $D^l_{mn}$ & $\Delta^l_{m[j]}$ \\\midrule
  0 & 0 & 0 \\
  1 & 0 & 0 \\
  2 & 0 & 0 \\
  3 & 2 & 1 \\
  4 & 3 & 1 \\
  5 & 0 & 0 \\
  6 & 7 & 2 \\
  7 & 4 & 1 \\
  8 & 5 & 1 \\
  9 & 8 & 2 \\\bottomrule
\end{tabular}
\caption{The number of non-vanishing $D^l_{mn}$ and linearly independent $\Delta^l_{m[j]}$ up to $l=9$, resulting from tetrahedral symmetry, for a fixed $m$. For a general inhomogeneous situation, $m=-l...l$, whereas in the flat wall geometry
(cylindrical symmetry), $m=0$.}
\label{tab:number_D}
\end{table}
\begin{table}[h]
\begin{tabular}{ccc}
\toprule
  $l$ & basis function & components \\\midrule
  3 & $\Delta^3_{m[1]}$ & $ \frac{1}{\sqrt 2} \wD^3_{m 2} + \frac{1}{\sqrt 2} \wD^3_{m \underline{2}}$ \\
  4 & $\Delta^4_{m[1]}$ & $ \frac{\sqrt 30}{12}\wD^4_{m \underline4} + \frac{\sqrt 30}{12} \wD^4_{m 4} -\frac{\sqrt 21}{6} \wD^4_{m 0}$ \\
  6 & $\Delta^6_{m[1]}$ & $ \frac{\sqrt 7}{4} \wD^6_{m \underline{4}} + \frac{\sqrt 7}{4} \wD^6_{m 4} + \frac{\sqrt 2}{4} \wD^6_{m 0} $  \\
      & $\Delta^6_{m[2]}$ & $- \frac{\sqrt{10}}{8} \wD^6_{m \underline{6}} + \frac{\sqrt{10}}{8} \wD^6_{m 6} -  \frac{\sqrt{22}}{8} \wD^6_{m\underline{2}} + \frac{\sqrt{22}}{8} \wD^6_{m 2} $ \\
  \bottomrule
\end{tabular}
\caption{Linear combinations of Wigner matrices that are invariant under all tetrahedral group transformations up to $l=6$
}
\label{tab:basis_fn}
\end{table}









\subsubsection{Tetrahedral symmetry}

Having chosen one of the conventions we can determine the Euler angles corresponding to every group element and then compute the "projection operator" 
from eq.~\eqref{eq:proj_op}. The necessary angles which enter the D-matrices are shown in \cref{tab:angles_T} for both patch conventions. Having chosen convention (B) we arrive at the following: $\pOp^{(1)} = \pOp^{(2)} = 0$, that means no Wigner matrices with $l=1, 2$ can appear in the expansion. Only starting with $l=3$ we start to see non-vanishing contributions to the expansion. Further, even though there are multiple non-vanishing moments for $l=\{3, 4\}$ in each case they are linearly dependent reducing the number of physically meaningful basis function to one.

The number of nonvanishing D-matrices as well as of the $\Delta$ invariants are shown in table~\ref{tab:number_D} normalized basis functions up to $l=6$ are shown in table~\ref{tab:basis_fn}



\subsubsection{Cylindrical symmetry (wall)}

Assuming cylindrical symmetry of the external potential perpendicular to the  $z$ axis (i.e. a flat wall) further reduces the number of non-vanishing moments. The external potential is now only $z$ dependent, hence
$\rho(\bm{r},\Omega)  \to \rho(z, \Omega)$. The density must now also be invariant under rotations of the molecule in the $xy$ plane (this leaves constant 
the distance of the individual patches with respect to the wall). These rotations correspond precisely to the final rotation (in reverse Euler order) with $\phi$ around the 
$Z$ axis. In other words we need
\begin{equation}
    \rho(z, \phi, \theta, \chi) = \rho(z, \phi + \delta , \theta, \chi) \qquad \forall \delta \in \left[0, 2\pi\right)
\end{equation}
which can only be achieved when $\rho$ does not depend on $\phi$. Hence only the moments $\rho^l_{0n}$ can be different from zero. 


\subsection{Pair potential in rotational invariants}
The anisotropic  part of the Kern-Frenkel potential can be expanded in so called rotational invariants \cite{gray84theory,blum1972invariant,ding2017efficient}
\begin{equation}
  \label{eq:kf_ex}
  V^{\text{KF}}(\bm{r}, \Omega_{1}, \Omega_{2}) = \sum_{m n l \mu\nu} V^{mnl}_{\mu \nu}(r) \Phi^{mnl}_{\mu \nu}(\Omega_{1}, \Omega_{2}, \hat{\bm{r}})
\end{equation}
The basis functions $\Phi^{mnl}_{\mu \nu}$ are a linear combination of D-matrices such that the projected coefficients $V^{mnl}_{\mu \nu}$ are independent of the choice for the fixed reference frame, hence
the name rotational invariants. They are given by \cite{gray84theory}
\begin{multline}
  \label{eq:28}
  \Phi^{mnl}_{\mu \nu}(\Omega_{1}, \Omega_{2}, \hbm{r}) = c_{m}c_{n}\sum_{\mu' \nu' \lambda'} \tj{m}{n}{l}{\mu'}{\nu'}{\lambda'}  \\ \times \conj{\wD^{m}_{\mu' \mu}}(\Omega_{1}) \conj{\wD^{n}_{\nu' \nu}}(\Omega_{2}) \conj{\wD^{l}_{\lambda' 0}}(\hat{\bm{r}})
\end{multline}
with $c_{n} = \sqrt{2n+1}$ and the Wigner $3j$ symbol which is a combinatorial quantity similar to Clebsch-Gordan coefficients but more intuitive symmetry properties.
In the definition of the basis function, the orientations of the two particles, and their separation vector factorize into different Wigner matrices. This means that we can change the orientation of one particle to a symmetrically equivalent one, without affecting the other particle or their separation vector. It is therefore easy to see how the symmetry properties of a single particle reduce the number of possible coefficients in the expansion of the pair potential. We replace the Wigner matrix for each particle in eq.~\eqref{eq:28} with the corresponding symmetrized basis function, {eq.~\eqref{eq:27}}. %

We thus obtain
\begin{multline}
 \label{eq:Phi_Delta}
    \Phi^{mnl}_{[ji]}(\Omega_{1}, \Omega_{2}, \hbm{r}) = c_{m}c_{n}\sum_{\mu' \nu' \lambda'} \tj{m}{n}{l}{\mu'}{\nu'}{\lambda'}  \\ \times \conj{\Delta^{m}_{\mu' [j]}}(\Omega_{1}) \conj{\Delta^{n}_{\nu' [i]}}(\Omega_{2}) \conj{\wD^{l}_{\lambda' 0}}(\hat{\bm{r}})
\end{multline}

From the basis function we derived before we see that the first non-vanishing pair potentials moments are
\begin{equation}
    \Phi^{330}_{[11]}, \Phi^{332}_{[11]}, \Phi^{334}_{[11]}, \ldots
\end{equation}
\tr{What is with 000, 030 etc.? Don't we need yet other symmetries like exchange to get these constraints?}


  
\subsection{Orientational density functional theory}


\subsubsection{General formalism}
\label{sec:dft_general}
The main objective of density functional theory is finding an analytical expression for the grand potential functional
$\Xi[\rho]$ which is a functional of the density profile $\rho(\bm{r}, \Omega)$. The equilibrium state is subsequently found by minimization
\begin{equation}
  \label{eq:18}
  \fdv{\Xi[\rho]}{\rho(\bm{r}, \Omega)} = 0\,,\quad \text{for } \rho = \rho_{\mathrm{eq}}(\bm{r}, \Omega)
\end{equation}
The grand potential functional is decomposed into an intrinsic free energy functional $\FE$ and
a one--body term involving  the external potential $V^{\text{ext}}$ and the chemical potential $\mu$:
\begin{equation}
  \label{eq:19}
  \Xi = \FE[\rho(\bm{r}, \Omega)] + \int \odif{\bm{r}} \odif{\Omega}\, \rho(\bm{r}, \Omega) \left[ V^{\text{ext}}(\bm{r},\Omega) - \mu \right]
\end{equation}
One can further split the free energy into an ideal, non-interacting term $\FE_{\text{id}}$ and the excess term $\FE_{\text{ex}}$ that results
from particle interactions
\begin{equation}
  \label{eq:20}
  \FE[\rho(\bm{r}, \Omega)] = \FE_{\text{id}}[\rho(\bm{r}, \Omega)] + \FE_{\text{ex}}[\rho(\bm{r}, \Omega)] \;.
\end{equation}
The first, ideal gas term is given by
\begin{equation}
  \label{eq:21}
   \FE_{\text{id}} = k_{B}T \int \odif{\bm{r}} \odif{\Omega}\, \rho(\bm{r}, \Omega) \left[\ln(\rho \Lambda^{3} K) -1  \right]
 \end{equation}
 and the second, excess term is in general unknown. {Here, $\Lambda$ is the thermal de-Broglie length.}
In order to separate the free energy contributions due to the orientation of the particles from the {orientation-independent} effects we split $\rho(\bm{r}, \Omega)$
into {an orientationally averaged} component $\rho(\bm{r})$ (depending only on $\bm{r}$) and an orientational distribution $\alpha(\bm{r}, \Omega)$
\begin{equation}
  \label{eq:product_ansatz}
  \rho(\bm{r}, \Omega) = \rho(\bm{r}) \alpha(\bm{r}, \Omega) \;.
\end{equation}
{The orientational distribution is normalized:}
\begin{equation}
  \label{norm_alpha}
  {\int d\Omega  \alpha(\bm{r}, \Omega)=1.}
\end{equation} 

The ideal part of the Helmholtz free energy in the anisotropic case becomes
\begin{multline}
  \label{eq:6}
  \beta \FE_{\text{id}} = \int \odif{\bm{r}} \rho(\bm{r}) \left[ \log(\Lambda^{3}\rho(\bm{r})) - 1 \right] \\
  + \int \odif{\bm{r}}\odif{\Omega}\, {\rho(\bm{r})} \alpha(\bm{r},\Omega) \log(K \alpha(\bm{r},\Omega))
\end{multline}
{We propose to split the excess free energy into an isotropic and an orientational part,}
\begin{equation}
  \label{eq:22}
\FE_{\text{ex}} = \FE_{\text{ex,iso}}[c] +  \FE_{\text{ex,or}}[\rho(\bm{r}), \alpha(\bm{r}, \Omega)]
\end{equation}
thus expecting that some parts of the free energy are entirely determined by the orientationally
averaged fluid density $\rho(\bm{r})$ alone (such as the hard-core interaction), while others will probably also need
information about the orientations of the particles. Anisotropic interactions of which the angular dependence was integrated out also fit into the first category.

By minizing the grand canonical ensemble $\Xi = \FE + \int \rho (V^{\text{ext}} - \mu)$ wrt the density $\rho(\bm{r})$ and the orientation distribution $\alpha(\bm{r}, \Omega)$
{ under the normalization constraint \eqref{norm_alpha}}
we arrive at the following Euler-Lagrange (EL) equations


\begin{multline}
\label{eq:2}
\rho(\bm{r}) = \exp \biggl( -\int \odif{\Omega}\, \alpha \log(K \alpha) + \beta \mu  \\ -\beta V^{\text{ext}} - \fdv{\beta \FE_\text{ex}[\rho,\alpha]}{\rho(\bm{r})} \biggr) 
\end{multline}
\begin{eqnarray}
    \label{eq:2b}
  \alpha(\bm{r}, \Omega)  &=& \frac{1}{\int \odif{\Omega}\, \psi(\bm{r}, \Omega) }\, \psi(\bm{r}, \Omega) \\
      & &  \psi(\bm{r}, \Omega) = \exp \left(-\frac{1}{\rho(\bm{r})}  \fdv{\beta \FE_\text{ex,or}[\rho,\alpha]}{\alpha(\bm{r}, \Omega)} \right) \;.  \nonumber
 \end{eqnarray}


\subsubsection{Existing isotropic functionals}

{The KF potential is the sum of an isotropic hard sphere part and anisotropic patch attractions. Therefore, it appears 
promising, in a first step, to treat also the free energy functional as a sum of an isotropic hard sphere reference part and a remainder accounting for the anisotropic interactions. 
The most accurate functionals for hard spheres are based on fundamental measure theory (FMT)\cite{roth2010fundamental}. 
Here, the excess free energy becomes a function of weighted densities $n_{\nu}(\bm{r})$ --- convolutions of the 
(orientationally averaged) particle density $\rho(\bm{r})$ with a set of geometry--based kernels.
It might seem surprising, that, in a second step, the anisotropic remainder can be approximated perturbatively with a functional depending
again only on the orientationally averaged particle density $\rho(\bm{r})$.
In the bulk, where the free energy only depends on the homogeneous bulk density, such a perturbation theory was 
developed by Wertheim (theory of associating fluids) for particles interacting attractively through $N_\mathrm{p}$ bonding sites \cite{wertheim1987thermodynamic}.
Only certain classes of bonding states are permitted which helps to restrict the possible number of configurations appearing in calculations, making an analytical treatment feasible. 
For treating inhomogeneous systems, the Wertheim bulk free energy needs to be ``functionalized'', and a first suggestion based 
on FMT has been given in Ref.~\cite{yuwu2002}. 
This functional has been further refined in \cite{stopper2018bulk} and has shown
rather good agreement with simulations at a medium to high temperature regime.}

{The sum of the hard sphere excess free energy (here taken as the original Rosenfeld functional) and the association part of
Ref.~\cite{stopper2018bulk} define $\FE_{\mathrm{ex,iso}}[\rho]$ in the free energy splitting of eq.~\eqref{eq:22}:}
\begin{equation}
  \label{eq:23}
  \beta \FE_{\mathrm{ex,iso}}[\rho] = \int \odif{\bm{r}} \left[ \Phi_{\mathrm{hs}}(\left\{ n_{\nu}(\bm{r}) \right\})  +
  \Phi_{\text{bond}}(\left\{ n_{\nu}(\bm{r}) \right\}) \right]
\end{equation}
\begin{multline}
  \label{eq:29}
  \Phi_{\mathrm{hs}}(\left\{ n_{\nu}(\bm{r}) \right\}) = -n_{0} \ln(1-n_{3}) \\
  + \frac{n_{1} n_{2} - {\bm{n}_{1}\cdot \bm{n}_{2}}}{1-n_{3}} + \frac{n_{2}^{3} - 3 n_{2} \bm{n}_{2}\cdot \bm{n}_{2}}
  {24 \pi (1-n_{3})^{2}}
\end{multline}
\begin{multline}
  \label{eq:24}
  \Phi_{\mathrm{bond}}(\left\{ n_{\nu}(\bm{r}) \right\}) = N_\text{p} n_{0}(\bm{r}) \xi^{q}(\bm{r}) \\
\times  \left[ \ln X(\bm{r}) - \frac{X(\bm{r})}{2} + 1/2 \right]
\end{multline}
{For the exact definitions of the weighted densities $n_\alpha(\bm{r})$, $\xi(\bm{r})$ as well as the space-dependent
bonding probability $X(\bm{r})$, we refer to Ref.~\cite{stopper2018bulk} (Sec. IIC therein).}






\subsubsection{Anisotropic mean field ansatz}
{A simple mean--field ansatz for the anisotropic part of the free energy functional is given by}
\begin{multline}
  \label{eq:25}
  \FE_{\text{ex}} = {\frac{1}{2}}\int \odif{\bm{r}_1}\odif{\bm{r}_2} \odif{\Omega_1} \odif{\Omega_2} \rho(\bm{r}_1)\alpha(\bm{r}_1, \Omega_1) \\ \times \rho(\bm{r}_2) \alpha(\bm{r}_2, \Omega_2) {V^{\text{MF}}}(\bm{r}_1 - \bm{r}_2, \Omega_1, \Omega_2)
\end{multline}
{This ansatz defines a yet unknown, orientation--dependent  mean--field potential $V^{\text{MF}}$ as the kernel. If one sets $V^{\text{MF}}=V^{\text{KF}}$, one obtains the standard RPA approximation for the anisotropic part in the KF fluid.
We expand both the orientations $\alpha(\bm{r}, \Omega)$ into the symmetrized basis functions $\Delta^b_{\beta' [j] }$,
\begin{equation}
   \alpha(\bm{r}, \Omega) = \sum_{b \beta' j}  \alpha^{b}_{\beta' [j]}  \Delta^b_{\beta' [j]}
\end{equation}    
as well as the mean-field potential,
\begin{equation}
   V^{\text{MF}}(\bm{r}, \Omega_{1}, \Omega_{2}) = \sum_{m n l [ij]} M^{mnl}_{[ij]}(r) \Phi^{mnl}_{[ij]}(\Omega_{1}, \Omega_{2}, \hat{\bm{r}}),
\end{equation}
where the $\Phi^{mnl}_{[ij]}$ are given by eq.~\eqref{eq:Phi_Delta}.  With these expansions, eq.~\eqref{eq:25} becomes}
\begin{multline}
  \label{eq:26}
  {\FE_{\text{ex}} = \frac{1}{2} \int \odif{\bm{r}_1}\odif{\bm{r}_2}   
  \rho(\bm{r}_{1})\rho(\bm{r}_{2}) } \sum_{AB}
  \alpha^{a}_{\alpha' [i]}(r_{1}) \alpha^{b}_{\beta' [j]}(r_{2}) \\
 \times \left[ \sum_{l \lambda'} M^{abl}_{[ij]}(r_{12}) \tj{a}{b}{l}{\alpha'}{\beta'}{\lambda'} D^{l}_{\lambda' 0}(\hat{\bm{r}}_{12})^* \right] \frac{64 \pi^{4}}{c_{a}c_{b}}
\end{multline}
with the sum over $A$ standing for $\sum_{a \alpha' i}$ and $B$ analogously. 
\begin{figure}[h]
  \centering
  \includegraphics[width=0.9\columnwidth]{wall_int}
\caption{Decomposition of the distance vector between two particles into components perpendicular and parallel to the wall. Due to the cylindrical symmetry we can integrate out $a_{12}$ and $\gamma_{12}$}
  \label{fig:cyl_integ}
\end{figure}

\subsubsection{Mean field with wall symmetry}
{For the KF fluid between flat walls, the cylindrical symmetry in the wall plane introduces further constraints on the expansion coefficients. 
As explained above, only orientation moments with a zero in the first lower index remain, $ \alpha^{b}_{\beta' [j]} \to  \alpha^{b}_{0 [j]} $, which also helps to reduce the number of contributing $3j$ symbols. 
Densities only depend on the $z$-coordinate (perpendicular to the walls), $\rho(\bm{r}) \to \rho(z)$, and the volume element 
is split as $d\bm{r}= dz d\bm{r}_{\parallel}$. The integral over the in-plane area element $ d\bm{r}_{1,\parallel}$ gives
$A$, the area of the wall. The second  in-plane area element $ d\bm{r}_{2,\parallel}= a_{12} d a_{12} d\gamma_{12}$ requires
integrations over the relative in-plane distance $a_{12}$ between points 1 and 2 as well as the relative azimuthal angle $\gamma_{12}$, see fig.~\ref{fig:cyl_integ}. 
We obtain}
\begin{widetext}
\begin{equation}
    \label{eq:rpa_wall}
    \FE_{\text{ex}} = {  \frac{A}{2} \int \odif{z_1} \odif{z_{2}} \odif{a_{12}} a_{12}  }  \odif{\gamma_{12}} \rho(z_{1})  \rho(z_{2})
    \sum_{AB}
    \alpha^{a}_{0 [i]}(z_{1}) \alpha^{b}_{0 [j]}(z_{2}) \left[ \sum_{l \lambda'} {M}^{abl}_{[ij]}(r_{12}) \tj{a}{b}{l}{0}{0}{\lambda'} \wD^{l}_{\lambda' 0}(\hat{\bm{r}}_{12})^* \right]  \frac{64 \pi^{4}}{c_{a}c_{b}}
    \end{equation}
\end{widetext}
{The distance between the two integration points is $r_{12} = \sqrt{a_{12}^2 + |z_1 - z_2|^2}$, and the orientation vector
$\hat{\bm{r}}_{12}=( \sin{\beta} \cos{\gamma_{12}},
 \sin{\beta} \sin{\gamma_{12}}, \cos\beta)^T $ is specified by the two angles $\beta = \arctan \frac{a_{12}}{(z_1 -z_2)}$ and $\gamma_{12}$. The appearing Wigner D-matrix with first lower index 0 is proportional to a spherical harmonic,
\begin{equation}
  \wD^l_{\lambda' 0}(\hbm{r}_{12}) = \sqrt{\frac{4\pi}{2 l+1}} Y^{\lambda'}_l  (\beta, \gamma_{12})\;.
\end{equation}
Thus one sees that} the integration over $\gamma_{12}$ gives the condition $\lambda' = 0$ and the D-matrix reduces to the Legendre polynomial
\begin{equation}
 \wD^l_{00}(\hat{\bm{r}}_{12}) = P_l(\cos \beta)=  P_l \left( \frac{z_1-z_2}{\sqrt{a_{12}^2 + |z_1 - z_2|^2}} \right)  .
\end{equation}
{Using this, the free energy in wall symmetry, eq.~\eqref{eq:rpa_wall}, is given by 
\begin{multline}
  \label{eq:fex_planar}
  \FE_{\text{ex}} =  \frac{A}{2}  \int \odif{z}\odif{z'} \rho(z) \rho(z') \\ \times \sum_{i'j'} \alpha^{i'}(z)   \alpha^{j'}(z') M^{i'j'}(z- z')
  \end{multline}
where the superindices $i',j'$ unite the indices of the $\alpha$-moments:
\begin{equation}
  \alpha^{a}_{0 [i]} \to \alpha^{i'}\;, \qquad  \alpha^{b}_{0 [j]} \to \alpha^{j'}\;, 
\end{equation}
and the reduced mean--field kernel $M^{i'j'}$ is given by
\begin{eqnarray}
  M^{i'j'}(z) &=& \sum_l \tj{a}{b}{l}{0}{0}{0}  \int \odif{a_{12}} a_{12}   M^{abl}_{[ij]}\left(\sqrt{a_{12}^2 + z^2}\right) \times \nonumber \\
  & & P_l \left( \frac{z}{\sqrt{a_{12}^2 + z^2}}\right)\;\frac{64 \pi^{4}}{c_{a}c_{b}} \;.
 \label{eq:kernel_reduced}
\end{eqnarray}
This result for the reduced mean--field kernel has important significance for the machine learning problem.
From simulation data in the flat wall geometry only the elements of $M^{i'j'}$  can be learned, up to a chosen cutoff
for the indices $i',j'$. However, these elements $M^{i'j'}$  only contain a subset of the moments $M^{abl}_{[\mu\nu]}$ for the  orientational invariants  of the full mean--field kernel, and moreover these in an integrated form, see eq.~\eqref{eq:kernel_reduced}. In perspective, this points to the necessity of including further types of external potentials, radially symmetric and orientation-dependent, into ML training procedures for learning a full mean--field kernel or kernels beyond mean field.}

{
However, in the RPA approximation the reduced mean--field kernel can be computed explicitly. We expand $V^\text{KF}$ (see eq.~\eqref{eq:16}) into symmetrized orientational invariants,
\begin{equation}
 V^{\text{KF}}(\bm{r}, \Omega_{1}, \Omega_{2}) = \sum_{m n l [ij]} V^{mnl}_{[ij]}(r) \Phi^{mnl}_{[ij]}(\Omega_{1}, \Omega_{2}, \hat{\bm{r}}),
\end{equation}
and project out the kernel moments $V^{mnl}_{[ij]}(r)$, obtaining:
\begin{align}
  V^{mnl}_{[ij]}(r) &= \epsilon^{mnl}_{[ij]} \phi_\text{sw}(r) \\
\epsilon^{mnl}_{[ij]} &=  \frac{2l+1}{256 \pi^5}\int \odif{\Omega_1} \odif{\Omega_2} \odif{ \hat{\bm{r}}_{12} } \conj{\Phi^{mnl}_{[ij]}} \\
& \times \sum_{\alpha,\beta=1}^{N_\text{p}}  \phi_{\text{patch}}(\bm{r}_{12}, \hat{\bm{r}}_{1}^{\alpha}(\Omega_{1}), \hat{\bm{r}}_{2}^{\beta}(\Omega_{2})) \nonumber 
\end{align}
The $r$--dependence is entirely in $\phi_\text{sw}(r)$, 
and the dependence on all indices is contained in the numbers $ \epsilon^{mnl}_{[ij]}$ which need to be computed numerically.
Then eq.~\eqref{eq:kernel_reduced} can be applied with $M \to V$. 
}













\subsubsection{Mean field ansatz for machine learning}
\label{sec:ansatz}

For the actual machine learning procedure, we use the free energy in eq.~\eqref{eq:fex_planar} with the kernel $M^{i'j'}(z)$
to be determined by ML. 
The superindices $i',j'$ contain an angular momentum--like index and a second index labelling the possible moments contributing for this agular momentum.
We allow all possible interactions between symmetric \tr{why symmetric?} moments up to certain number $l$ for the angular momentum--like index. Apart from being a practical necessity, we also observe that with increasing $l$ the moments become smaller, further providing a rationale for this cutoff. 
We chose to include moments up to $l<6$ as extracting moments with low enough noise for higher $l$ from simulation data proved to be increasingly time-consuming. Additionally, due to symmetry, moments with $l=5$ vanish, leaving us with just two nonvanishing
superindices $=3,4$ as there is only one moment for these $l$ (see also tab.~\ref{tab:basis_fn}) . 

Furthermore, since we want to learn a functional for the orientational part $\FE_{\text{ex,or}}$ of the free energy 
(see Sec.~\ref{sec:dft_general}), we  specifically exclude interactions that only depend on two zero moments, i.e. $M^{00}$, such that the bulk behavior (where the orientational distrubution becomes isotropic) remains untouched. 
Thus the general form of the mean field ansatz for  $\FE_{\text{ex,or}}$ for the ML problem is
\begin{multline}
\label{eq:11}
    \FE_{\text{ex,or}}^\text{mf} = \frac{A}{2} \int \odif{z}\odif{z'} \rho(z) \rho(z') \\ \times 
    \sum_{\substack{i,j \\ \text{not }i=j=0}} \alpha^i(z)   \alpha^j(z') M^{ij}(z- z')
  \end{multline}
where the indices $i$ and $j$ are the angular momentum--like indices $\{0,3,4\}$.
From eq.~\eqref{eq:rpa_wall} we can deduce the symmetry properties of the mean field interaction potentials for negative distances, which are shown in table~\ref{tab:sym_mf}.

\begin{table}[h]
\centering
\begin{tabular}{cc}
\toprule
  $M^{ij}$ & parity \\\midrule
  (0, 3) & odd \\
  (0, 4) & even \\
  (3, 3) & even \\
  (3, 4) & odd \\
  (4, 4) & even \\\bottomrule
\end{tabular}
\caption{Symmetry properties of the mean field potentials under inversions around the origin}
\label{tab:sym_mf}
\end{table}
Taken together with the fact that 
\begin{equation}
    M^{ij}(-z) = M^{ji}(z)
\end{equation}
we reduce the total number of independent mean field potentials to the five shown in table~\ref{tab:sym_mf}.
Further, the potentials are assumed to be translationally invariant, i.e. they only depend on the distance between the moments
thus the integrals reduce to convolutions which can be performed efficiently using the fast Fourier transform.


The density functional derivative of this mean field functional is
\begin{multline}
  \label{eq:fdv_rho}
 \fdv{ \FE_{\text{ex,or}}^\text{mf}[\rho,\alpha]}{\rho(z)} %
 \\ \sum_{i, j} \alpha^i(z)  \left[ \rho \alpha^j  \ast M^{ij} \right] + \alpha^j(z) \left[ \rho \alpha^i  \ast \overline{M}^{ij} \right]
\end{multline}
where $\overline{M}(z)$ = $M(-z)$ and the symbol $\ast$ denotes a convolution. 
For the equation that determines the orientation distribution, we need the derivative w.r.t. the individual moments
\begin{equation}
  \label{eq:fdv_alpha}
   \fdv{  \FE_{\text{ex,or}}^\text{mf}[\rho,\alpha]} { \alpha^k(z)} = \rho(z) \left[ \rho \alpha^j \ast M^{kj} \right] + \rho(z) \left[\rho \alpha^i \ast \overline{M}^{ik} \right]
\end{equation}

As a consequence of the mean field ansatz, it turns out, that the self-consistent equation for the density, eq.~\eqref{eq:2}, can be further simplified. 
Upon using eqs.(\ref{eq:2b},\ref{eq:2c}), the entropic contribution of the orientation distribution in eq.~\eqref{eq:2}  becomes
\begin{multline}
    -\int \odif{\Omega}\, \alpha(z,\Omega) \log(K \alpha(z, \Omega)) 
     =  \log  \frac{1}{K} \int \odif{\Omega} \psi(z, \Omega) \\ +
    \int \odif{\Omega}\, \alpha(z, \Omega) \frac{2l+1}{K} \conj{\wD^l_{mn}}(\Omega) \frac{1}{\rho(z)} \fdv{\beta \FE^\text{mf}_\mathrm{ex,or}[\rho, \alpha]}{\alpha^l_{mn}}
\end{multline}
Plugging in our solution from \cref{eq:fdv_alpha} and comparing to \cref{eq:fdv_rho} shows that the term on the right hand side cancels the contribution of $\delta \FE_{\text{ex,or}}^\text{mf}/\delta \rho$ in the Euler-Lagrange equation \eqref{eq:2} which
becomes:
\begin{equation}
 \label{eq:rho_ML}
\rho(z) = \frac{\int \odif{\Omega}\, {\psi(z,\Omega)} }{K} \exp \biggl(   \beta \mu  \\ -\beta V^{\text{ext}} - \fdv{\beta \FE_\text{ex,iso}[\rho]}{\rho({z})} \biggr) 
\end{equation}
This is inherent to the mean field ansatz and as a consequence we can not fit $\FE^\text{mf}_\text{ex,or}$ to correct the differences between our reference functional and the simulation data. The only change the orientation distribution induces on the density is through the multiplicative first term on the rhs of eq.~\eqref{eq:rho_ML}
which is already fixed by the observed orientation distribution $\alpha(z, \Omega)$ and turns out to be rather small as we will later see.
Nonetheless, this simplified approach is a valuable starting point for further more sophisticated models.

\section{KF model calculations: training data and reference model results}

\begin{figure}%
  \centering
  \includegraphics[width=.9\columnwidth]{phasediag}
  \caption{Phase diagram for the Wertheim theory based reference functional. In the cross section of the shaded $T^*$ and $\eta$ intervals, training data have been generated. The blue data points correspond to the state points for the orientational moments shown in \cref{fig:ori_data} and the red crosses to those of the density profile comparison in \cref{fig:wall_bond}. The black marker shows the location of the critical temperature and the line corresponds to the coexistence-line between the gas and liquid phase.}
  \label{fig:phasediag}%
\end{figure}

Parameters for the KF system were chosen as $N_\text{p}=4$, $\delta=0.119$ and $\cos \theta = 0.895$. For these parameters,
the critical point was determined in ref.~\cite{foffi2007possibility} with coordinates $\rho_c^*= \rho_c\sigma^3 = 0.267$
($\eta_c = (\pi/6)\rho_c^* = 0.140 $) and $T_c^* = (kT)/\epsilon = 0.1682$, using simulations. 

\subsection{Reference functional results}

The gas-liquid coexistence curve resulting from the reference functional \eqref{eq:23} is the one from Wertheim theory for associating liquids and can be found in 
ref.~\cite{stopper2019structure}, fig. 3.3. The critical temperatures from Wertheim theory and simulations match quite well but there is a discrepancy in $\eta_c$, see fig.~\ref{fig:phasediag}. Note, however, that the binodal is very flat in the vicinity of the critical point such that the simulation critical point is very close to the reference binodal.
In Fig.~\ref{fig:wall_bond}, we show profiles $\rho(z)$ of the averaged density at a hard wall obtained from the reference
functional and simulations. 
\tr{Perhaps more data: Three $T^*=0.2,0.24,0.3$ for $\rho^*=0.19$ (critical density of Wertheim) and $\rho^*=0.27$
(critical density of sim).\tb{added} These should be without the anisotropy correction.}
see \cref{fig:kf_comparison_more}.
As one can see from the figures, the lower the temperature gets, the worse is the agreement between theory and simulation. It is clear, that preferred particle orientations start to become more and more important in shaping the fluids behavior.
\tr{Depending on the results, some more remarks...}


\begin{figure}[t]
  \centering
    \includegraphics[width=\columnwidth]{kf_comparison_more.pdf}
  \caption{Comparison of data obtained through simulation of the KF model (full line) with those that result from the excess free energy in eq.~\eqref{eq:23} (dashed line), at the bulk densities $\rho_b = 0.19$  (left) and $\rho_b = 0.27$ (right) for different temperatures.}
  \label{fig:kf_comparison_more}
\end{figure}


\subsection{Simulations}
In order to obtain the necessary training data of the orientation distributions, we
simulated the system as a canonical Monte Carlo simulation (constant $NVT$ ensemble), using a code from Rovigatti et al., described in ref.~\cite{rovigatti2018simulate}. The code was suitably modified to incorporate hard walls at distance $L_\text{w}$ with
their normal in $z$--direction. Initial configurations are generated by randomly 
placing particles into the simulation box. The number of particles was
fixed to $N=1000$ and the length of the cubic simulation box is hence
$L=\left( N/\rho \right)^{1/3}$. After the initial thermalization phase we 
save a sample of the system every 400 MC sweeps.
For training state points we chose temperatures $ T^* \in \{0.20;0.22;0.26;0.30\} $  and bulk densities $\rho^* \in \{0.10;0.13;0.16;0.19;0.21;0.24;0.27\} $. See also fig.~\ref{fig:phasediag} for the location of the training points in the
phase diagram.

\begin{figure}[t]
  \centering
    \includegraphics[width=\columnwidth]{kf_comparison.pdf}
  \caption{Comparison of data obtained through simulation of the KF model (simulation) with those that result from the excess free energy in eq.~\eqref{eq:23} (reference), at different bulk densities and reduced temperatures.}
  \label{fig:wall_bond}
\end{figure}





From equilibrated samples, profiles $\rho(z)$ of the averaged density are obtained by standard histograms and orientation profiles are obtained according to eqs.~\eqref{eq:expansion_coeff} and \eqref{eq:product_ansatz} as follows
\begin{equation}
  \label{eq:alpha_hist}
  \alpha^l_{m[j]}(z_i) = \frac{1}{\rho(z_i)} \frac{2l + 1}{K} \sum_{\Omega_k \in z_i} \Delta^l_{m[j]}(\Omega_k)
\end{equation}
where $z_i$ labels the bin the particle is in and $\Omega_j$ is the orientation of the $j$th particle in bin $z_i$.








\begin{figure}%
  \centering
  \includegraphics[width=\columnwidth]{oris_comparison}
  \caption{The first two non-trivial orientational moments extracted from the simulation data for different temperatures and densities as defined by \eqref{eq:alpha_hist}. Both $\alpha^i$ were multiplied by $K = 8 \pi^2$}
  \label{fig:ori_data}%
\end{figure}



In the limit of $T^*\to\infty$ the KF model reduces to the hard sphere model and there is no anisotropy in the density profiles.
With decreasing temperature however, the bonding mechanism becomes more important and changes the orientational distribution of the fluid near the wall, see Fig.~\ref{fig:ori_data}. \tr{Also here we should think to plot a $T^*$ series for one density at least. Let us have a look and see what we have. }\tb{added}
A comparison of the strength of the orientations for different temperatures is shown in \cref{fig:ori_data_same_density} 

We observe, that the temperature dependence of the orientational moments is not very strong (in the chosen parameter range), but nonetheless visible. \tb{seems quite strong actually}

\begin{figure}%
  \centering
  \includegraphics[width=\columnwidth]{oris_comparison_same_density.pdf}
  \caption{Here we show the both orientational moments separately for different temperatures and the bulk densities $\rho_b = 0.13$ (left) and $\rho_b = 0.27$ (right). 
  The upper panels show $\alpha^3$ and the lower ones $\alpha^4$}
  \label{fig:ori_data_same_density}%
\end{figure}







\section{Machine learned DFT}

Our goal is to find out whether it is possible to determine the potentials $M^{ij}$ such that solving the fix point (FP) equation for the orientation
gives us results that are similar to those of Monte Carlo simulations of the system.
As shown earlier, due to the mean field ansatz, the EL equation for the density is only minimally coupled to 
the solution of the orientation distribution.
This permits us to reduce the problem to only solving the FP equation \eqref{eq:2b} for $\alpha(z, \Omega)$.
The immediate question now is, which density to use when evaluating the excess free energy derivative on the right-hand
side. Were we to solve the full problem with a completely general $\FE_\text{ex}$, this would ideally be the density resulting from the Monte Carlo simulation 
of the model that we try to reproduce with DFT. But as the mean field ansatz doesn't have the capability to correct
the difference w.r.t. to our reference bonding functional, for now we use the densities produced by just the reference functional.
We will be using a machine learning framework to find the correct mean field potentials. In fact, Machine Learning has been used before in the context of
classical DFT to find a (symbolic) expression for the excess free energy of a 1D hard-rod and a Lennard-Jones system \cite{shang2019classical}.
There, the self-consistency of eq.~\eqref{eq:2} was exploited to find the ideal parameters $\theta$ of the network. In other words
\begin{equation}
  \rho(\bm{r}; \theta)_\text{ML} = \exp \left( \beta \mu - \beta V^\text{ext}  - \beta \fdv{\FE^\mathrm{ex}[\rho; \theta]}{\rho(\bm{r})}_{\rho_\mathrm{eq}}\right)
\end{equation}
with the loss function
\begin{equation}
  L(\theta) = \int \odif{\bm{r}} \left( \rho(\bm{r}; \theta)_\text{ML} - \rho_\text{eq}(\bm{r}) \right)^2
\end{equation}
We are going to use a similar approach for the orientation distribution functions.
To make matters a little clearer we rewrite the above fix point condition as
\begin{equation}
  \label{eq:phi_root}
    \Phi(\rho; \theta) = f(\rho_\text{eq}; \theta) - \rho
\end{equation}
with $f$ depending also on $\beta, \mu$ and $V^\text{ext}$,
such that the learned solutions (which depends on the parameters $\theta$ of the network) becomes the root of $\Phi$
\begin{equation}
    \rho(\bm{r}; \theta)_\text{ML} = \Root \Phi(\rho; \theta)
\end{equation}
The solution of the orientation distribution has the same structure. In this case, where the excess free energy also
depends on the orientation, $\alpha$ enters as an additional argument
\begin{equation}
    \Psi(\rho, \alpha; \theta) = g(\rho_\text{eq}, \alpha_\text{eq}; \theta) - \alpha
\end{equation}
Note, that the inputs to the functions $f$ and $g$ can in this case be the equilibrium values because during the training
the solutions $\rho_\text{ML}$ and $\alpha_\text{ML}$ are supposed to approach these values and should become 
equal ideally.

Suppose now we found a good set of parameters $\theta$ that fulfill the above requirement. Our aim was to use
the learned functional to quickly find physical solutions of the Kern-Frenkel model at different thermodynamic points
without needing to do a time-consuming Monte Carlo simulation. This requires again solving the roots of $\Phi, \Psi$ only this time
not knowing the true equilibrium values of the density and orientation distribution. In other words, we need to \emph{simultaneously} find the roots of
\begin{gather}
\Phi(\rho, \alpha; \theta) = f(\rho, \alpha; \theta) - \rho \\
\Psi(\rho, \alpha; \theta) = g(\rho, \alpha; \theta) - \alpha
\end{gather}
Such equations are usually solved iteratively, starting from an initial guess $\rho_\text{init}, \alpha_\text{init}$.
Sensible values are the bulk density and the isotropic orientation distribution $\alpha(z, \Omega) = 1/K$.
It is evident however, that now the determination of the root is more complicated compared to before (during training)  as the inputs to $f, g$ vary during every step (expect for $\theta$, which is fixed now) and
it is not necessarily given that this time they converge to the same solution as before.

An additional complication compared to the case treated in \cite{shang2020FEQL} is that this time our training data
cannot be produced by an exact functional but must be collected from MC simulations and therefor contains some
amount of noise. When training the network as in eq.~\eqref{eq:phi_root} we need to solve for the root up to a rather high relative error
as we only have information of the function at the physical fixed point itself. But when the equilibrium data is noisy, as it is in our case, this becomes problematic and we are eventually over-fitting, leading to an unphysical solution. 


One way to alleviate these problems is to complete the whole fixed point finding procedure also during the training step, starting from intial values that are far from equilibrium values. The resulting solutions are
then automatically self-consistent.
While  this is in principle possible, there are some drawbacks, mainly due to
the fact that we need to store the complete computational graph with intermediate value in order to be able to back-progate through the loss and find
better parameters $\theta$. The memory consumption grows with the number of iteration steps that we do to find the root and hence we are going to be
limited to some maximum number of steps that we can do.
The further we are from the solution, the more steps are usually necessary, so one could keep memory consumption low by
starting the root finding procedure from a point not too far from the equilibrium.
Another approach that is gaining popularity in the machine learning community is using implicit differentiation during the backward pass.
It allows one to compute the gradient w.r.t. loss without retaining the complete computational graph necessary to find the fix point. The knowledge of
the fix point is enough to compute the gradient $\nabla_\theta(\cdot)$, so one can use \emph{any} method to compute the fix point without the need of storing intermediate values.

In our case this approach would translate to the following. We initialize the parameters $\theta_0$, e.g. by setting them to zero. We then find the root
of $\Psi(\rho, \alpha; \theta_0)$, starting from the intial values $\rho_\text{init}$ and $\alpha_\text{init}$. Under the assumption that the iteration converges, we arrive at the fix point $\alpha_0(z, \Omega)$, where the index reminds us of the fact that this solution depends on $\theta_0$. Different from the previous strategy, the FP might very well
be something completely different from our sought solution $\alpha_\text{eq}$. What we gained however, is the certainty that $\alpha_0$ is indeed a self-consistent solution during the whole iterative process. Making use of implicit differentiation we can compute $\nabla_\theta \ell$, where
\begin{equation}
  \label{eq:fp_loss}
  \ell = \MSE \left[ \alpha_0, \alpha_\text{eq} \right]
\end{equation}
and use this value in our optimizer to arrive at a better value $\theta_1$ and so on.

One drawback of this approach is that during the backward pass it is necessary to compute the matrix inverse of the Jacobian of the forward transformation. This is due to how automatic differentiation works internally.
Assume that $\alpha^\star$ is a fixed point of $g(\alpha; \theta)$, and we're interested in how the fixed point changes upon changing the parameters of the network. Using the implicit function theorem we have
\begin{equation}
  \label{eq:31}
  \pdv{\alpha^\star}{\theta} = \pdv{g}{\theta}_{\alpha^\star} \left[ \mathbb{I} - \pdv{g}{\alpha}_{\alpha^\star} \right]^{-1}
\end{equation}
The inverse on the r.h.s. is usually solved iteratively but depending on the function $g$ and the fixed point we are momentarily at, the solution might become increasingly expensive,
numerically unstable or even non-existent. One proposed method to alleviate this problem are so-called \emph{Phantom Gradients}. The idea is to expand the Jacobian inverse in a Neumann series and truncate after the first term. This corresponds to replacing the inverse with the identity matrix~\cite{geng2021training}. Translated into our training procedure this means the following. We still find the fixed point
solution $\alpha^\star$ for a certain set of parameters $\theta$, however we don't take the computations into account when constructing the computational graph\footnote{Using for example \texttt{Tensor.detach()} or \texttt{jax.lax.stop\_gradient(x)} in the two popular ML packages PyTorch and JAX}. Since we know that this point is a fixed point up to a certain tolerance we can plug it back into the function $g$ and use this computation for the backward pass. Apart from being much faster it has been shown to improve the stability of the training \cite{chang2022object,geng2021training}
 

The forward step is performed as follows.
Training data consists of a set $\{\rho(z), \alpha^{3}(z) \equiv \alpha^{3}_{0[1]}, \alpha^4(z) = \alpha^{4}_{0[1]}\}$ for every bulk density and temperature.
The potentials $M^{ij}(z)$ in eq.~\eqref{eq:fdv_rho} and \eqref{eq:fdv_alpha} are parametrized by $M$ variables each, which correspond to their value in real space on a grid from $-L/2$ to $L/2$ with spacing $\Delta z$. As the spacing $\Delta z$ for the potentials is different from the spacing of the training data points we need to translate from one support to the other. This is
done by linear interpolation of the potentials to every $z$ axis in the data set.

The generative step consists of
\begin{enumerate}
  \item Evaluating the non-normalized orientation distribution by
  \begin{align*}
    \psi(z,\Omega;\theta)  = \exp \left(\frac{1}{\rho(z)} \sum_{lmn}\fdv{\beta \FE_{\mathrm{ex}}[\rho,\alpha;\theta]}{\alpha^{l}_{m[j]}(z)} \conj{\Delta^{l}_{m[j]}}(\Omega) \frac{2l + 1}{K} \right)
  \end{align*}
  \item Normalizing $\alpha(z,\Omega;\theta) = \psi(z,\Omega;\theta)/\int\odif{\Omega} \psi(z,\Omega;\theta)$
  \item Projecting out the moments of interest
  \begin{align*}
    \alpha^{l}_{m[j]}(z;\theta) = \frac{2l+1}{K} \int \odif{\Omega} \alpha(z,\Omega;\theta) \conj{\Delta^{l}_{m[j]}}(\Omega)
  \end{align*}
\end{enumerate}

    




\subsection{Learned potentials}

When parameterizing convolution kernels or in this case potentials directly in real space they tend to become rather noisy during training due to the stochastic nature of the optimization
and the fact that we interpolate the potentials onto the support of the training data sets. To reduce the noisiness we ``coarse grain'' the potentials by defining them on a grid with larger spacing $\Delta z$
compared to the spacings of the training data.
Further, in order to regularize the kernels we also add a $L^1$ penalty (absolute value norm) term to the loss
\begin{equation}
  \label{eq:tot_loss}
  \ell = \MSE \left[ \alpha^\star, \alpha_\text{eq} \right] + \lambda \sum_{ij} L^1(M^{ij})
\end{equation}
The stronger the parameter $\lambda$, the more expensive it becomes for the network use non-zero kernel values and hence create interactions between the moments. If the regularizer is too large we expect
to get a bad reproduction of the orientational moments, whereas for values of $\lambda$ too small, the kernels are overfitting on the noise that is
present in the training data.
In order to find the ideal values of $M$ and $L$ we did a hyperparameter-optimization with $M \in [64, 128]$, $\lambda \in [10^{-1}, 10^{-2}, \ldots, 10^{-7}, 0]$ and $L \in [4.0, 6.0]$. We observed that the final loss does not vary
strongly with the parameters $L$ and $M$. The resulting kernels are smoother for the small $M$ but some resolution is lost in interesting regions like inside the sphere $r < \sigma/2$.


In fig.~\ref{fig:aa_pot} we show a set of resulting potentials for different values of $\lambda$. One can nicely see, how with decreasing $\lambda$ more and more interaction terms emerge and as a consequence the orientational moments improve, as shown in fig.~\ref{fig:aa_results}. It is surprising to see that relatively few interactions
between orientational moments are already capable of describing most of the angular structure that is present.
By the nature of the mean field ansatz we expect it work better at higher temperatures. This can indeed be observed when we look at the results for lower temperatures as shown in \cref{fig:aa_results1,fig:aa_results14}.
In both high- and low-density case the predicted orientations are slightly weaker than observed in simulations. One can also see however, that between the two, the higher-density system is described more accurately, presumably because the hard-core interaction is more present in this case weakening any complicated angular interactions.

\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{kernels_comparison}
  \caption{The learned potentials with decreasing regularizer $\lambda$. The other parameters were $L=6$ and $M=128$. The last set of potentials starts to show unphysical contributions from long-range interactions due to noisy data.}
  \label{fig:aa_pot}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{results_comparison}
  \caption{Self-consistent solutions of the orientational part of the EL equations, computed with the learned potentials shown in fig.~\ref{fig:aa_pot}. The second picture already shows good agreement, while the step from third to fourth adds only a small amount of accuracy in the peaks. The state point is at $T=0.24$ and $\rho_b = 0.19$}
  \label{fig:aa_results}
\end{figure}


\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{results_comparison_idx1}
  \caption{Self-consistent solutions for the orientational moments at the state point $T=0.20$ and $\rho_b = 0.13$}
  \label{fig:aa_results1}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{results_comparison_idx14}
  \caption{Self-consistent solutions for the orientational moments at the state point $T=0.20$ and $\rho_b = 0.27$}
  \label{fig:aa_results14}
\end{figure}


\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figures/isotherm_comparison_3.pdf}
  \caption{Resulting potentials trained on different isotherms but same regularizer $\lambda$}
  \label{fig:aa_results14}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figures/isotherm_comparison_5.pdf}
  \caption{}
  \label{fig:aa_results14}
\end{figure}

\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{figures/isotherm_comparison_7.pdf}
  \caption{}
  \label{fig:aa_results14}
\end{figure}


The learned interaction potentials show an interesting structure. Looking at the third panel in \cref{fig:aa_pot} (chosen for good performance in describing the orientation and for readability),
we observe repulsion inside the sphere region for the moment pairs $(0, 4)$ and $(3, 3)$. Rather localized at the edge of the sphere we see a repulsion between $(3, 4)$ and again further outside
at around $z=1$ for the pairs $(0, 3)$ and $(0, 4)$. Attraction is only seen between the pairs $(0, 3)$ and $(0, 4)$, both containing as one partner the isotropic density, i.e. $\rho(r) \alpha^0$.



\subsection{Applications}

\tb{? Extrapolation to higher density/temp?}






\section{Summary and outlook}






\bibliography{mybibliography} 
\end{document}

